gyre_tides: Modeling binary tides within the gyre stellar oscillation code

We describe new functionality in the GYRE stellar oscillation code for modeling tides in binary systems. Using a multipolar expansion in space and a Fourier-series expansion in time, we decompose the tidal potential into a superposition of partial tidal potentials. The equations governing the small-amplitude response of a spherical star to an individual partial potential are the linear, non-radial, non-adiabatic oscillation equations with an extra inhomogeneous forcing term. We introduce a new executable, gyre_tides, that directly solves these equations within the GYRE numerical framework. Applying this to selected problems, we find general agreement with results in the published literature but also uncover some differences between our direct solution methodology and the modal decomposition approach adopted by many authors. In its present form gyre_tides can model equilibrium and dynamical tides of aligned binaries in which radiative diffusion dominates the tidal dissipation (typically, intermediate and high-mass stars on the main sequence). Milestones for future development include incorporation of other dissipation processes, spin-orbit misalignment, and the Coriolis force arising from rotation.

==> New gyre_tides (Copy)/symbols.tex <==
%% Constants & units

\newcommand{\Msun}{M_{\odot}}
\newcommand{\Rsun}{R_{\odot}}
\newcommand{\Lsun}{L_{\odot}}

\DeclareSIUnit\dyne{dyn}
\DeclareSIUnit\year{yr}

%% Binary system properties

\newcommand{\Mpri}{M}
\newcommand{\Rpri}{R}
\newcommand{\Lpri}{L}

\newcommand{\mratio}{q}

\newcommand{\vpos}{\mathbf{r}}
\newcommand{\vsec}{\mathbf{r}_{2}}
\newcommand{\rsec}{r_{2}}

\newcommand{\vex}{\mathbf{e}_{x}}
\newcommand{\vey}{\mathbf{e}_{y}}
\newcommand{\vez}{\mathbf{e}_{z}}
\newcommand{\ver}{\mathbf{e}_{r}}
\newcommand{\vet}{\mathbf{e}_{\vartheta}}
\newcommand{\vep}{\mathbf{e}_{\varphi}}
\newcommand{\vei}{\mathbf{e}_{i}}

\newcommand{\thetasec}{\theta_{2}}
\newcommand{\phisec}{\varphi_{2}}

\newcommand{\tanom}{\upsilon}
\newcommand{\eanom}{\mathcal{E}}
\newcommand{\manom}{\mathcal{M}}
\newcommand{\tperi}{t_{0}}
\newcommand{\phiperi}{\varphi_{0}}

\newcommand{\Oorb}{\Omega_{\rm orb}}
\newcommand{\Porb}{P_{\rm orb}}

\newcommand{\Operi}{\Omega_{\rm peri}}
\newcommand{\Ops}{\Omega_{\rm ps}}

\newcommand{\epstide}{\varepsilon_{\rm T}}

\newcommand{\sigmk}{\sigma_{m,k}}

%% Stellar structure

\newcommand{\Teff}{T_{\rm eff}}

\newcommand{\Lrad}{L_{\rm R}}
\newcommand{\epsnuc}{\epsilon}

\newcommand{\cP}{c_{P}}
\newcommand{\nablaad}{\nabla_{\rm ad}}
\newcommand{\upsT}{\upsilon_{T}}

\newcommand{\kapad}{\kappa_{\rm ad}}
\newcommand{\kapS}{\kappa_{S}}
\newcommand{\epsad}{\epsilon_{\rm ad}}
\newcommand{\epsS}{\epsilon_{S}}

\newcommand{\vOrot}{\mathbf{\Omega}_{\rm rot}}
\newcommand{\Orot}{\Omega_{\rm rot}}
\newcommand{\Opsy}{\Omega_{\rm ps}}

\newcommand{\vFrad}{\mathbf{F}_{\rm rad}}
\newcommand{\Fradr}{F_{{\rm rad},r}}
\newcommand{\vFcon}{\mathbf{F}_{\rm con}}

\newcommand{\tdyn}{t_{\rm dyn}}
\newcommand{\tthm}{t_{\rm thm}}

\newcommand{\rs}{r_{\rm s}}

%% Tidal formalism

\newcommand{\Slamb}{S_{\ell}}

\newcommand{\potpri}{\Phi}
\newcommand{\potsec}{\Phi_{2}}
\newcommand{\pottide}[1][0]{\Phi_{{\rm T}\if#10\else;#1\fi}}
\newcommand{\pottot}[1][0]{\Psi\if#10\else_{#1}\fi}

\newcommand{\vxi}{\boldsymbol{\xi}}
\newcommand{\xir}{\xi_{\rm r}}
\newcommand{\xit}{\xi_{\vartheta}}
\newcommand{\xip}{\xi_{\varphi}}

\newcommand{\xih}{\xi_{\rm h}}
\newcommand{\vxih}{\vxi_{\rm h}}

\newcommand{\vv}{\mathbf{v}}

\newcommand{\angtime}[1][0]{H_{\if#10\else#1\fi}}

\newcommand{\txir}[1][0]{\tilde{\xi}_{{\rm r}\if#10\else;#1\fi}}
\newcommand{\txih}[1][0]{\tilde{\xi}_{{\rm h}\if#10\else;#1\fi}}

\newcommand{\tf}[1][0]{\tilde{f}_{\if#10\else#1\fi}}
\newcommand{\tP}[1][0]{\tilde{P}_{\if#10\else#1\fi}}

\newcommand{\tpotpri}[1][0]{\tilde{\potpri}_{\if#10\else#1\fi}}
\newcommand{\tpottot}[1][0]{\tilde{\Psi}_{\if#10\else#1\fi}}
\newcommand{\tpottide}[1][0]{\tilde{\Phi}_{{\rm T}\if#10\else;#1\fi}}

\newcommand{\trho}[1][0]{\tilde{\rho}_{\if#10\else#1\fi}}
\newcommand{\tS}[1][0]{\tilde{S}_{\if#10\else#1\fi}}
\newcommand{\tT}[1][0]{\tilde{T}_{\if#10\else#1\fi}}

\newcommand{\tFradr}[1][0]{\tilde{F}_{{\rm rad},r\if#10\else;#1\fi}}

\newcommand{\teps}[1][0]{\tilde{\epsilon}_{\if#10\else#1\fi}}
\newcommand{\tkap}[1][0]{\tilde{\kappa}_{\if#10\else#1\fi}}
\newcommand{\tLrad}[1][0]{\tilde{L}_{{\rm R}\if#10\else;#1\fi}}

\newcommand{\cbar}[1][0]{\bar{c}_{\if#10\else#1\fi}}
\newcommand{\Fbar}[1][0]{\bar{F}_{\if#10\else#1\fi}}
\newcommand{\Gbar}[2][0]{\bar{G}^{(#2)}_{\if#10\else#1\fi}}
\newcommand{\gbar}[1][0]{\bar{\gamma}_{\if#10\else#1\fi}}

\newcommand{\kap}[1][0]{\kappa_{\if#10\else#1\fi}}

\newcommand{\torque}{\mathcal{T}}
\newcommand{\angmom}{\mathcal{J}}

\newcommand{\torsec}{\torque_{\rm sec}}

\newcommand{\tcirc}{t_{e}}

\newcommand{\pf}{\mathcal{R}}

\newcommand{\detune}{\epsilon}
\newcommand{\ndetune}{\bar{\detune}}

\newcommand{\overlap}{Q_{n,\ell}}

%% Oscillations

\newcommand{\gmode}[1]{{\rm g}_{#1}}

\newcommand{\signl}{\sigma_{n,\ell}}
\newcommand{\gamnl}{\gamma_{n,\ell}}

%% GYRE implementation

\newcommand{\mS}{\mathsf{\mathbf{S}}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vzero}{\mathbf{0}}

%% Math symbols

\newcommand{\real}{\operatorname{Re}}
\newcommand{\imag}{\operatorname{Im}}

\newcommand{\ee}[1]{\operatorname{e}^{#1}}
\newcommand{\ii}{\mathrm{i}}

\newcommand{\diff}[1]{\operatorname{d}\!{#1}}
\newcommand{\deriv}[3][0]{\frac{\operatorname{d}\if#10\else^{#1}\!\fi\!{#2}}{\operatorname{d}\!{#3}\if#10\else^{#1}\fi}}
\newcommand{\sderiv}[3][0]{\operatorname{d}\if#10\else^{#1}\fi\!{#2}/\operatorname{d}\!{#3}}
\newcommand{\pderiv}[3][0]{\frac{\partial\if#10\else^{#1}\!\fi{#2}}{\partial{#3}}}
\newcommand{\spderiv}[3][0]{\partial\if#10\else^{#1}\fi{#2}/\partial{#3}}

\newcommand{\nablah}{\nabla_{\rm h}}

%% Codes

\newcommand{\gyre}{GYRE}
\newcommand{\mesa}{MESA}
\newcommand{\cafein}{CAFein}

\newcommand{\xgyre}{\texttt{gyre}}
\newcommand{\xgyretides}{\texttt{gyre\_tides}}

%% Text

\newcommand{\BV}{Brunt-V\"ais\"al\"a}

%% Editing

\newcommand{\edited}[1]{\textbf{#1}}

